The Lambda Calculus is Quantifiable

In this paper we introduce several quantitative methods for the lambda-calculus based on partial metrics, a well-studied variant of standard metric spaces that have been used to metrize non-Hausdorff topologies, like those arising from Scott domains. First, we study quantitative variants, based on program distances, of sensible equational theories for the $\lambda$-calculus, like those arising from B\"ohm trees and from the contextual preorder. Then, we introduce applicative distances capturing higher-order Scott topologies, including reflexive objects like the $D_\infty$ model. Finally, we provide a quantitative insight on the well-known connection between the B\"ohm tree of a $\lambda$-term and its Taylor expansion, by showing that the latter can be presented as an isometric transformation.

==> section2.tex <==
The Scott topology is widely used in computer science because it captures a notion of computability via continuity.

It is regrettably not Haussdorf: if $x < y$, any open set including x must also contain y.

On the opposite side, every topology induced by a metric must be Haussdorf.

Hence, the Scott topology is often seen as a "bizzare" topology, far away from the topological intuitions one can get from metric spaces.

But, it is known, in the litterature \val{citation}, that by relaxing certain conditions on the notion of metric, one can still capture a notion of distance while inducing non-Haussdorf topology.

This is what we discuss in this section.

\val{Est-ce qu'on devrait citer le theoreme qui dit que on capture TOUT avec les quantales ?}

\begin{definition}[Bestiary of Metrics]
	We consider functions on a space $X$ of the form $p:X\times X\to [0,\infty]$.
	
	Such a function is a \emph{partial pseudo metric} (PPM) when it satisfies the following axioms:
	
	\begin{description}
		\item[Symmetry] $p(x,y) = p(y,x)$
		\item[Small self distances (SSD)] $p(x,x) \leq p(x,y)$
		\item[Triangularity] $p(x,z) + p(y,y) \leq p(x,y) + p(y,z)$
	\end{description}

		Such a metric induces a preorder on $X$: $x \leq_p y$ when $p(x,y) \leq p(x,x)$.
	
		Notice that this implies by (SSD) that $p(x,y) = p(x,x)$
		
		This preorder in turn induces an equivalence $\simeq_p$
	
	A \emph{partial metric} (PM) is a PPM satisfying:
	
	\begin{description}
		\item[Equality] If $p(x,x) = p(x,y) = p(y,y)$ then $x=y$
	\end{description}
	
	In that case, $<_p$ is an order, ie $\simeq_p$ is equality.

	
	A \emph{partial ultra-metric} (PUM) on a space $X$ is a $PMS$ where the \emph{Triangularity} axiom is replaced by the stronger:
	
	\begin{description}
		\item[Ultra] For all $z$, $p(x,y)\leq \max\{p(x,z),p(z,y \}$
	\end{description}

	Finally, a \emph{pseudo metric} is a metric in the usual sense, but without the axiom:
	
	\begin{description}
		\item[Exact] $p(x,y) = 0 => x = y$
	\end{description}

	In particular, a pseudo metric $p$ is a partial metric. It's preorder $\leq_p$ is an equivalence.

	We will say that a metric \emph{captures} an order when it's induced order is said order.
\end{definition}

\begin{example}\label{interval}
	The closed intervals of $\mathbb{R}$, noted $\intv$, form a PMS with partial metric: $\delta(I_1, I_2) := inf \{ |b-a| | I_1 \cup I_2 \subseteq [a, b]\}$, which is the size of the smallest intervals containing $I_1$ and $I_2$.
	
	The order defined by the metric here is intuitive, it is reverse inclusion / the scott information order: $x \leq y$ iff $p(x,y) \leq p(x,x)$ iff $y \subseteq x$. The more information one has, the higher.
	
	This example explains the choice of the word "partial": an interval, in term of Scott topology, represents an information on a partial execution: we have yet to discover the precise real number that we are computing. By contrast, the total elements will be the one with self distance $0$ (so the one where $p$ is like a regular metric), ie of the form $\{r\}$, a complete information, of a terminated execution.
\end{example}

\begin{example}[Simple Examples]
	
	\begin{itemize}
		\item The Sierpinski space can be equipped with a partial metric $s$ $s(0,0)=s(0,1)=1$, $s(1,1)=0$.
		
		The unique non-empty balls here are $\{1\}$ and $\{0,1\}$
		
		\item The euclidean metric is a metric hence a partial metric. It's order is the equality on real numbers.
		
		\item On $\mathbb{R}$ one can define the partial ultrametric $u(r,s)=2^{-\min\{r,s\}}$. Notice that $u(r,r)=2^{-r}$.
		The order $\leq_u$ coincides with the order of real numbers: $2^{-\min\{r,s\}}=2^{-s}$ iff $s=\min\{r,s\}$ iff $s\leq r$.
		
	\end{itemize}
\end{example}

The following lemma will be very useful:
\val{citer Myronyk ou HVZ au final ?}
\cite{Myronyk2022}
\begin{lemma}[cf.~\href{https://www.sciencedirect.com/science/article/pii/S0166864117303772?ref=pdf_download&fr=RR-2&rr=81ec0c76bb2ba264}{HVZ2017}]
	For any partial metric $p: X\times X\to [0,\infty]$ there exists a \emph{$1$-bounded} partial metric $p^{\leq 1}:X\times X\to [0,\infty]$, defined by $p^{\leq 1}(x,y) := \frac{p(x ,y)}{1+p(x,y)}$
	such that $\C O_{p}(X)= \C O_{p^{\leq}}(X)$.
\end{lemma}

\begin{proposition}
	A partial pseudo metric $p$ induces a pseudo metric $d_p(x,y) := 2p(x,y) - p(x,x) - p(y,y)$. This pseudo metric has the property that $x \simeq_p y$ iff $x \simeq_{d_p} y$.
	
	With $x \simeq_{d_p} y := d_p(x,y) = 0$ 
\end{proposition}

\subsection{Tree Partial Metric}

%(IMPORT FROM SECTION. 3)

\pao{- tree partial metric (from Section 3): also mention the more standard tree metric, say that the latter does not capture the Scott topology (for the Hausdorff reason) while we will show that the former does}

Let us introduce the \emph{tree partial metric}: this metric will capture the scott topology, while the usual tree metric does not. \val{laquelle exactement ? je trouve pas de reference meme si je crois que je vois}

 Let $\Sigma\mathrm{Tree}_{\leq\infty}$ be the set of (non necessarily finite) finitely branching, $\Sigma$-labeled trees, where $\Sigma$ is a countable set of labels.
For any $\alpha\in\Sigma \mathrm{Tree}_{\leq\infty}$, let $|\alpha|\in \mathbb N\cup\{ \infty\}$ indicate the \emph{height} of $\alpha$. Moreover, for any $n\in \mathbb B$, let $\alpha_n$ be the finite tree obtained by truncating all paths of $\alpha$ at length $n$, if $|\alpha| \geq n$, and be indefinite otherwise. We write $\alpha_n \downarrow=\beta_n $ to indicate that $\alpha_n$ and $\beta_n$ are both definite and equal, and $\alpha_n \downarrow\neq\beta_n $ to indicate that either one of $\alpha_n$ and $\beta_n$ is indefinite, or they are both definite and distinct. 
%Moreover, let $\ell_n(\alpha,\beta)\in\{0,1\}$ be $0$ if $\alpha_n \downarrow=\beta_n $ or if
%either one of $\alpha_n$ and $\beta_n$ is indefinite, and be $1$ is $\alpha_n \neq\beta_n$. 

\begin{definition}[tree partial metric]
	For any $\alpha, \beta\in\Sigma \mathrm{Tree}_{\leq\infty}$, let 
	\begin{align*}
		\mathrm{div}(\alpha,\beta)&:=\min \{ n \mid \alpha_n \downarrow=\beta_n \ \land \  \alpha_{n+1}\downarrow\neq\beta_{n+1}    \}, \\
		p_{\mathrm{tree}}(\alpha,\beta)&:= 2^{-\mathrm{div}(\alpha,\beta)},
		%\\
		%p^\ell_{\mathrm{tree}}(\alpha,\beta)&:= 2^{-\mathrm{div}(\alpha,\beta)}+\ell_\mathrm{div}(\alpha,\beta)(\alpha,\beta),
	\end{align*}
	where it is intended that $2^{-\infty}=0$. 
\end{definition}


$p_{\mathrm{tree}}$ is a partial ultrametric over $ \mathrm{Tree}_{\leq\infty}$. Notice that, for a finite tree $\alpha$, its self-distance is $p_{\mathrm{tree}}(\alpha, \alpha)=2^{-|\alpha|}$, and that $p_{\mathrm{tree}}(\alpha, \alpha)=0$ iff $\alpha$ has infinite height. In the next sections we will show that $p_{\mathrm{tree}}$ captures the Scott topology on $ \mathrm{Tree}_{\leq\infty}$.

==> section4.tex <==
We now want to extend our model from a model of simply typed lambda calculus to a model of untyped lambda calculus.

For this, we will mimic the usual $D_{\infty}$ construction of Scott \val{citation needed} of a reflexive object, but we will in parallel build a partial metric for the result.

Let $(D, \leq, p)$ be a partial metric domain. We first recall the construction of the domain $D_{\infty}$:

For each $n$, let the domain $D_{n}$ be defined by 
\begin{align*}
	D_{0}&:= D, \\
	D_{n+1}&:= \C C(D_{n}, D_{n}).
\end{align*}
We define injection-projection pairs $(i_{n},j_{n}): D_{n} \to_{ip}D_{n+1}$ by
\begin{align*}
	i_{0}(x)&:= \lambda y.x & j_{0}(f)&= f(\bot) \\
	i_{n+1}(f)&= i_{n}\circ f\circ j_{n}& 
	j_{n+1}(g)&= j_{n}\circ g\circ i_{n}.
\end{align*}

%The domain $D_{\infty}$ is defined as 
%$$
%D_{\infty}=\left \{ x \in \prod_{n \in 0}^{\infty}\bigcup_{n}D_{n} \Big \vert \forall n\in \BB N, x_{n}\in D_{n} \ \land \
%x_{n}=j_{n}(x_{n+1})\right\}.
%$$

\val{J'ai change la def, je comprenais pas la tienne ?}

The domain $D_{\infty}$ is defined as 
$$
D_{\infty}=\left \{ x \in \prod_{n = 0}^{\infty} D_{n} \Big \vert \forall n\in \BB N, x_{n}=j_{n}(x_{n+1})\right\}.
$$

For all $m<n$ (say $n=m+q$) we can define maps $i_{mn}:D_m\to D_n$ and
$j_{nm}:D_n\to D_m$ via
\begin{align*}
	i_{m(m+1)}&:= i_m &   j_{(m+1)m}&:= j_m \\
	i_{m(m+q+2)}&:= i_{(m+1)(m+1+q)}\circ i_m &
	j_{(m+q+2)m}&:=
	j_{(m+1)m}\circ j_{(m+q+2)(m+1)}
\end{align*}

%% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRABEB9AWxAF9S6TLnyEUARnJVajFmy7BuAanF9+gkBmx4CRAExTq9Zq0QgAOuYDGUCDgQCh20UQDMhmSfmdgYALSq6k4iuigALB7GcmYKYGp80jBQAObwRKAAZgBOELyIZCA4EEiSIABGMGBQSK4FDHQVDAAKwjpiIFhg2LAgRrKmHT7c8RrZuSXURUgG5ZXViLV9XmZYQypq1PWNLc6hHV1YPY4gY3kzUwvUFVU1BVEDq75+ehsgWzDNrS4rB0ejOXl3IViogIrMbgs7v02I9-IFNg0PjsQu1Ot1WMdTkgChcwdd5otPNFBoo4r03ojPrt2gwYBkcEETgCkGCLkD8bcEdsvns0YdWEtiQArHxwkaZZmXYHTK5zTlEgYip4vRlYxDnEGlDmQwWKtaBTGS0oXArawnvKkomG-AUKthK4bkuAACyw9OxhvGoMmINNcp1FO51LYtPduvtosdCT4QA
%\begin{tikzcd}
%	D_m \arrow[r, "i_{m}" description, bend left] \arrow[rrrr, "i_{mn}", bend left] & D_{m+1} \arrow[r, "i_{m+1}" description, bend left] \arrow[l, "j_{m}" description, bend left] & \cdots \arrow[r, "i_{n-2}" description, bend left] \arrow[l, "j_{m+1}", bend left] & D_{n-1} \arrow[r, "i_{n-1}" description, bend left] \arrow[l, "j_{n-2}", bend left] & D_{n} \arrow[l, "j_{n-1}" description, bend left] \arrow[llll, "j_{nm}", bend left]
%\end{tikzcd}

Moreover, we can define maps
$i_{n\infty}:D_n \to D_\infty$ and 
$j_{\infty n}:D_\infty \to D_n$ via
\begin{align*}
	(i_{n\infty}(x))_k&:=
	\begin{cases}
		j_{nk}(x)
		&
		n=k+q
		\\
		x
		&
		k=n
		\\
		i_{nk}(x)
		& k= n+q
	\end{cases}
\end{align*}
and
$$
j_{\infty n}(x):= x_n.
$$

Here are diagrams summing up the situation:

\val{Je sais pas pourquoi il rend mal sur internet c'est pas colle comme ça}

%%%
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRABEB9AWxAF9S6TLnyEUARnJVajFmwA68gMZQIOBAKHY8BIgCYp1es1aIOnQn2kwoAc3hFQAMwBOEXojIgcEJJJAARjBgUEgAzF4MdEEMAArCOmIgWGDYsCBGsqbJnMDcfPyCIK7uftQ+SAaBwaGIEZkmbFi5YAC04gXUUTHx2qJNqVjpmsVuHlUViP5BIeFexnJmAFYt7Z0g3TBxCf1mKWms1HAAFlhOOEjEIyUe-pNeM7X1G9FbvSK6e4PpDYsgK3l1iczhdPNcxpdyr5EFVHkgACwATl+2WaeTA6022z6nxALiwtmOF3BpRhUMh1VmiCRKLYALA+QyLx6O1x+MJxIofCAA
\begin{tikzcd}
	D_m \arrow[r, "i_{m}" description, bend left] \arrow[rr, "i_{mn}"', bend left=49] & \cdots \arrow[r, "i_{n-1}" description, bend left] \arrow[l, "j_{m}" description, bend left] & D_n \arrow[l, "j_{n-1}" description, bend left] \arrow[ll, "j_{nm}"', bend left=49]
\end{tikzcd}

% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZAFgBoAGAXVJADcBDAGwFcYkQAPAAgB0eswXACIB9ANYgAvqXSZc+QigBMFanSat2AKxHAxAW0kAKDgEpe-QaOCGpMkBmx4CRAGyqaDFm0QgsusTBjMwsBYV0gu1knBSIARg91b3Y+AGMoCBwEaWj5FxQAZkSvTV80jKyohzlnRWQAVmKNHxByzOz7Rzy6gHYm5LKedPaqrtqiMji1EpbrPgEAMxwAT0lRmtiUcn7SzhF5sCXlrgBeKTUYKABzeCJQBYAnCH0kPpAcCCRtpN2+NH8JDRGPQAEYwRgABQ2+RAjBgSxANDBYCgSAK5ByIEezy+NA+ryRMBRaO+wLBkOhilh8JwiJ+LW4fA+XA4ugORzWkkokiAA
\begin{tikzcd}
	x_\infty = & \cdots & j_{km}(x) \in D_{m} & \cdots & x \in D_k \arrow[d, "x \to x_{\infty}", bend left] & \cdots & i_{kn}(x) \in D_{n} & \cdots \\
	&        &                     &        & D_{\infty} \arrow[u, "\pi_k", bend left]           &        &                     &       
\end{tikzcd}

Observe that in $D_{\infty}$ we have that $x\ll y$ iff there exists $N\in \BB N$ such that 
$
x \leq \bigvee_{n\leq N}i_{n\infty}(y_{n})\ll y$.
This is an immediate consequence of the remark that $y=\bigvee_{n=0}^{\infty}i_{n\infty}(y_{n})$.

\val{Je suis aller voir Amadio Curien, c'est  Remark 3.1.9, cette preuve est incomprehensible, leur abus de notation est affreux on ne comprend meme pas lenonce}

\medskip

\val{ref les sections precedentes}

By Theorem \ref{th:exponential} each domain $D_{n}$ is a partial metric domain via any of the metrics $p^\lambda_{n}$ (for $0<\lambda \leq \frac{1}{2}$) defined by
\begin{align*}
	p^\lambda_{0}&= p \\
	p^\lambda_{n+1}(f,g)&= \sum_{i=1}^{\infty}\lambda^i p_{n}(f(a_{i}),g(a_{i})),
\end{align*}
where $a_{i}$ ranges over a fixed countable basis of $D_{n}$.



\subsection{$D_\infty$ is quantifiable}

We define the metrics $p_n:D_n\times D_n\to [0,+\infty]$ by induction as follows:

\begin{align*}
	p_0(x,x')& = p(x,x'), \\
	p_{n+1}(x,x')&= p_{D_n\To D_n}^{\frac{1}{2^n}} (x,x')= \sum_{k=1}^{\infty}\frac{1}{2^{nk}}p_n(x(w^n_k), x'(w^n_k)).
\end{align*}

\begin{remark}\label{pncapturesscott}
	Since the $w^n_k$ form a basis of $D_n$, thanks to Theorem \ref{th:exponential}, the metric $p_{n+1}$ generates the Scott topology of $D_{n+1}$.
\end{remark}


\begin{lemma}\label{lemmall1}
	For all $n\in \BB N$ and $x,y\in X_n$, $x\ll y$ implies $i_n(x)\ll i_n(y)$.
	
\end{lemma}
\begin{proof}
	Let $D\subseteq X_{n+1}$ be a directed set such that 
	$i_n(y)\leq \bigvee D$. 
	Let $jD=\{ j_n(d)\mid d\in D\}\subseteq X_n$. Let us show that $jD$ is directed: 
	given $j_n(d_1), j_n(d_2)\in jD$, $i_n(j_n(d_1))\leq d_1$ and 
	$i_n(j_n(d_2))\leq d_2$; now, since $D$ is directed, there exists $d_3\in D$ with 
	$d_1,d_2\leq d_3$; observe that this implies
	$j_n(d_1), j_n(d_2)\leq j_n(d_3)$. Since $j_n(d_3)\in jD$ we can conclude that $jD$ is directed.
	
	From $i_n(y)\leq \bigvee D$ we deduce
	that 
	$y=j_n(i_n(y))\leq j_n(\bigvee D)= \bigvee jD$, where in the last step we use the fact that $ j_n$ is continuous. Now, from $x\ll y$ it follows that $ x\leq j_n(d)$ holds for some $d\in D$, and thus
	$i_n(x)\leq i_n(j_n(d))\leq d$. We can thus conclude that 
	$i_n(x)\ll i_n(y)$.
\end{proof}


\begin{lemma}\label{lemmall22}
	For all $n\in \BB N$, $x\in X_n$ and $y\in X_\infty$, 
	$x \ll y_n$ $\To$ $i_{n\infty}(x)\ll y$.
	
\end{lemma}
\begin{proof}
	
	Suppose $x\ll y_n$. Let us first show that 
	$i_{n\infty}(x)\leq y$.
	First, from $x\leq y_n$ we deduce $i_{n(n+q)}(x)\leq i_{n(n+q)}(y_n)=
	i_{n(n+q)}(j_{(n+q)n}(y_{n+q}))
	\leq y_{n+q}$.
	Moreover, from $x\leq y_n$ we also deduce
	$j_{n(n-q)}(x)\leq j_{n(n-q)}(y_n)=y_{n-q}$. Hence, for all $q\in \BB N$, 
	$(i_{n\infty}(x))_q\leq y_q$, which implies $i_{n\infty}(x)\leq y$. 
	
	
	Suppose now $D\subseteq X_\infty$ is a directed set such that $y\leq \bigvee D$. Let $D_n=\{d_n\mid d\in D\}$. Recall that $d_n=j_{\infty n}(d)$. 
	Let us show that $D_n$ is directed: let $j_{\infty n}(d_1),j_{\infty n}(d_2)\in D_n$, then 
	$i_{n\infty}(j_{\infty n}(d_1))\leq d_1$ and 
	$i_{n\infty}(j_{\infty n}(d_2))\leq d_2$ and since $D$ is directed there exists $d_3\in D$ such that $d_1,d_2\leq d_3$. Then we have that 
	$j_{\infty n}(d_1),j_{\infty n}(d_2)\leq j_{\infty n}(d_3)$ and, since 
	$ j_{\infty n}(d_3)\in D_n$, this shows that $D_n$ is directed as well.
	
	
	Now, since $d_n=j_{\infty n}(d)$ and $j_{\infty n}$ is continuous, 
	from $y\leq \bigvee D$ we deduce
	$y_n \leq j_{\infty n}(\bigvee D)= \bigvee D_n$. 
	From $x\ll y_n$ we conclude then that there exists $ j_n(d)\in D_n$ such that 
	$x\leq j_n(d)=d_n$. 
	
	To prove that $  i_{n\infty}(x)\leq d$, let us show that for all $k\in \BB N$, 
	$( i_{n\infty}(x))_k\leq d_k$: if $k=n$,
	$( i_{n\infty}(x))_k = x\leq d_n=d_k$; if $k< n$, then 
	$( i_{n\infty}(x))_k = j_{nk}(x)$ and from 
	$x\leq d_n$ we deduce 
	$( i_{n\infty}(x))_k=j_{nk}(x)\leq j_{nk}(d_n)=d_k$; finally, if $k>n$, 
	$( i_{n\infty}(x))_k = i_{nk}(x)$ and from 
	$x\leq d_n$ we deduce 
	$( i_{n\infty}(x))_k=i_{nk}(x)\leq i_{nk}(d_n)=i_{nk}(j_{kn}(d_k))\leq d_k$.
\end{proof}


\begin{lemma}\label{lemmall3}
	For all $x,y\in X_\infty$, $x\ll y$ iff there exists $N\in \BB N$ and 
	$w_1,\dots,w_k\in X_{N}$ such that
	$$
	w_1,\dots, w_k \ll y_N
	$$
	and
	$$
	x \leq  i_{N\infty}(w_1\vee\dots\vee w_k)
	$$
	
\end{lemma}
\begin{proof}
	Let $D$ be the set of all $i_{n\infty}(w_n)\in X_n$, for some $n\in \BB N$, such that $
	w_n \ll y_n$.
	Observe that, by Lemma \ref{lemmall22}, any $i_{n\infty}(w_n)\in D$ satisfies $i_{n\infty}(w_n)\leq y$. This implies that all finite joins of elements of $D$ exist in $X_\infty$.
	Let $D^*$ be the set of all such finite joins. Notice that $D^*$ is directed since $d,d'\in D^*$ implies $d\vee d^*\in D^*$. 
	
	Since a base for $X_\infty$ is formed by elements of the form $i_{n\infty}(b)$, here $b$ is in the base of $X_n$, and since $X_\infty$ is a continuous domain, we deduce that 
	$y\leq \bigvee D\leq \bigvee D^*$. 
	
	Now, from $x\ll y\leq \bigvee D^*$, since the $D^*$ is directed, we deduce that there exists finitely many elements $u_1, \dots, u_k$ of $D$, where $u_j\in X_{n_j}$, such that 
	$x \leq i_{n_1\infty}(u_1)\vee\dots\vee i_{n_k\infty}(u_k)$. 
	To conclude it suffices to let $N=\max\{n_j\mid j=1,\dots,k\}$ and let
	$w_j:= i_{n_jN}(u_j)$, by observing that 
	(1) $u_j\ll y_{n_j}$ implies $w_j\leq y_N$ by Lemma \ref{lemmall1} and (2) 
	$ i_{n_j\infty}(u_j)=
	i_{N\infty}(i_{n_jN}(u_j))=i_{N\infty}(w_j)$.
\end{proof}

\begin{lemma}\label{lemmall2}
	For all $n\in \BB N$, $x\in X_n$ and $y\in X_\infty$, 
	$i_{n\infty}(x)\ll y$ $\To$ $\exists N\forall k\geq N, i_{n(n+k)}(x)\ll y_{n+k}$;
	
	
\end{lemma}
\begin{proof}
	
	From $i_{n\infty}(x)\ll y$ via Lemma \ref{lemmall3} we deduce that there exists 
	$M\in \BB N$ and $w_1, \dots, w_k\in X_{N}$ such that 
	$w_j\ll y_M$ and 
	$i_{n\infty}(x) \leq  i_{M\infty}(w_1\vee\dots\vee w_k)$, where we can suppose that 
	$n\leq M$.
	
	
	Let $N=M-n$. 
	Since $i_{n\infty}(x)=i_{M\infty}(i_{nM}(x))$, from 
	$i_{n\infty}(x) \leq  i_{M\infty}(w_1\vee\dots\vee w_k)$ we deduce
	$i_{n(n+N)}(x)= (i_{n\infty}(x))_M\leq w_1\vee\dots\vee w_k\ll y_{M}$.
	
	
	Finally, to conclude that $i_{n(n+k)}(x)\ll y_{n+k}$ holds for all $k\geq N$ we can argue by induction, using Lemma \ref{lemmall1} and the fact that $i_{m}(y_m)\leq y_{m+1}$. 
	
	
\end{proof}


%%%% This is the important part of the section

Define the distance on $D_\infty$ as 
$$
p_\infty(x,x'):=\sum_{n=1}^\infty\frac{1}{2^n}p_n(x_n, x'_n).
$$

\metricscott
\begin{proof}
	\begin{description}
		\item[$\C O_\sigma(D_\infty)\supseteq\C O_{p_\infty}(D_\infty)$:]
		
		Let $y\in B_\epsilon(x)$. We need to find $y'\in D_\infty$ such that $y'\in B_\epsilon(x)$ and 
		$y'\ll y$. 
		
		
		From $p_{\infty}(y,x)<p_{\infty}(x,x)+\epsilon$ ift follows that we can find $\theta, \delta>0$ such that 
		$p_{\infty}(y,x)<p_{\infty}(x,x)+\delta$ and $\delta+\theta\leq \epsilon$.
		
		Let $N$ be such that $\sum_{n>N}^\infty\frac{1}{2^n}< \frac{\theta}{2}$. 
		For all $n\leq N$, we can find some $z_n\in B_{\frac{\theta}{2}}(y_n)$ such that 
		$z_n\ll y_n$ by \ref{pncapturesscott}.
		
		Observe that by Lemma \ref{lemmall22} we have $i_{n\infty}(z_n)\ll y$.
		This implies in particular since the cpo is bounded complete, that the join $\bigvee_{n=1}^N i_{n\infty}(z_n)$ exists in $D_\infty$.
		
		Define $y':= \bigvee_{n=1}^N i_{n\infty}(z_n)$. Notice that $y'\ll y$ holds so we just have to check that 
		$y'\in B_\epsilon(x)$.
		

		First recall that, by antimonotonicity of $p_n$, $p_n(a\vee a', b)\leq \min\{p_n(a,b), p_n(a',b)\}$.
		
		Now, for all $n\leq N$, we have that $y'_n=j_{\infty n}(y')=\left( \bigvee_{k<N}i_{k,n}(z_k)\right ) \vee z_n \vee
		\left( \bigvee_{n<k\leq N}j_{k,n}(z_k)\right)$. Then we deduce $p_n(y'_n,y_n)\leq p_n(z_n, y_n)< p_n(y_n,y_n)+ \frac{\theta}{2}$.
		
		
%				First recall that, by monotonicity of $p_n$, $p_n(a\vee a', b)\leq \max\{p_n(a,b), p_n(a',b)\}$.
%		Moreover, from $p_n(z_n, y_n)\leq \epsilon$ it follows, by monotonicity \val{expliciter via la prop de Dinfini et lajonction} of $p_n$ and Proposition \ref{propnonexp}, that 
%		$p_{n+q}(i_{n(n+q)}(z_n), y_{n+q})\leq
%		p_{n+q}(i_{n(n+q)}(z_n), i_{n(n+q)}(y_{n}))\leq
%		p_n(z_n, y_n)\leq \frac{\theta}{2}$. 
%		
%		Putting these two facts together we can deduce that for all $n\leq N$, $p_n(y'_n, y_n)\leq \frac{\theta}{2}$. 
		
		
		We can now compute
		\begin{align*}
			p_\infty(y',x)&= \sum_{n=1}^\infty\frac{1}{2^n}p_n(y'_n, x_n) \\
			&\leq
			\sum_{n=1}^\infty\frac{1}{2^n}\Big( p_n(y'_n, y_n)+p_n(y_n, x_n)-p(y_n,y_n) \Big )\\
			&\leq
			\left(\sum_{n=1}^\infty\frac{1}{2^n} p_n(y'_n, y_n)-p_n(y_n,y_n)  \right) +p_\infty(y,x)\\
			&= \left(\sum_{n=1}^N\frac{1}{2^n} (p_n(y'_n, y_n)-p_n(y_n,y_n))\right) +\left( \sum_{n>N}^\infty\frac{1}{2^n} (p_n(y'_n, y_n)-p_n(y_n,y_n)) \right)+p_\infty(y,x)\\
			&< \left(\sum_{n=1}^N\frac{1}{2^n}\frac{\theta}{2}\right) + \frac{\theta}{2} +p_\infty(x,x) +\delta\\
			&\leq p_\infty(x,x)+\theta+\delta\\
			&\leq p_\infty(x,x)+\epsilon.
		\end{align*}
		
		%From $ p_\infty(y,x)\leq \epsilon$ it follows that $p_0(y_0,x_0)\leq \epsilon$, whence 
		%$y_0\in B_\epsilon(x_0)$. Since $B_\epsilon(x_0)$ is Scott-open, there exists
		%$y'_0\in B_\epsilon(x_0)$ such that $y'_0\ll y_0$.
		%
		%Let $y':= i_{0\infty}(y'_0)$. 
		%We can conclude that $y'\ll y$ by using Lemma \ref{lemmall2} $ii.$, since 
		%$y'=i_{0\infty}(y'_0)$.
		%Let us show by induction that for all $n$, $y'_n\in B_\epsilon(y_n)$:
		%this is true by definition for $n=0$; if $n=m+1$, then from
		%$y'_m\in B_\epsilon(y_m)$ we deduce $p_m(y'_m, y_m)\leq \epsilon$, and by Proposition \ref{propnonexp} $p_m(i_m(y'_m), i_m(y_m))\leq \epsilon$, that is
		%$p_n(y'_n, i_m(y_m))\leq \epsilon$. Since $y_m= j_m(y_n)$, we have that 
		%$ i_m(y_m)=i_m(j_m(y_n))\leq y_n$, and by monotonicity of $p_m$ we can conclude
		%$p_n(y'_n, y_n)\leq \epsilon$.
		%
		
		
		
		\item[$\C O_\sigma(X_\infty)\subseteq\C O_{p_\infty}(X_\infty)$]
		
		Suppose $ x\ll y$. We need to find $\epsilon>0$ such that $B_\epsilon(y)\subseteq\ \twoheaduparrow x$.
		By Lemma \ref{lemmall3} there exists $N$ and 
		$w_1, \dots, w_k\in X_{N}$ such that
		$
		x \leq  i_{N\infty}(w_1\vee\dots\vee w_k)\ll y
		$.
		By Lemma \ref{lemmall2} there exists $N'\geq N$ such that
		$
		i_{NN'}(w_j) \ll y_{N'}
		$. 
		
		Observe that $i_{N'\infty}(i_{NN'}(u))= i_{N\infty}(u)$, which implies that \\  
		$x \leq \bigvee_j  i_{N'\infty}(i_{NN'}(w_j) )  $.
		
		
		
		For each $j=1,\dots, k$ we can find then $\epsilon_j>0$ such that 
		$B_{\epsilon_j}(y_{N'})\subseteq \ \twoheaduparrow i_{NN'}(w_j)$.
		
		
		Let $\epsilon:= 2^{-(N'+1)}\min\{\epsilon_j\mid j=1,\dots, k\}$.
		Suppose $z\in B_\epsilon(y)$: for all $j=1,\dots,k$, from $p_\infty(z,y)\leq \epsilon$ we deduce
		$p_{N'}(z_{N'}, y_{N'})\leq 2^{N'}\epsilon < \epsilon_j$, whence 
		$z_{N'}\in B_{\epsilon_j}(y_{N'})$, which forces
		$i_{NN'}(w_j) \ll z_{N'}$. 
		
		By Lemma \ref{lemmall22}  the last inequality implies 
		$i_{N'\infty}(w_j)=i_{N'\infty}(i_{NN'}(w_j) )\ll z$, and we thus obtain
		$x \leq  \bigvee_j  i_{N'\infty}(i_{NN')}(w_j) ) \ll z$, that is, $x\ll z$.
	\end{description}
\end{proof}




